Meta-Learned Confidence for Few-shot Learning

Transductive inference is an effective means of tackling the data deficiency problem in few-shot learning settings. A popular transductive inference technique for few-shot metric-based approaches, is to update the prototype of each class with the mean of the most confident query examples, or confidence-weighted average of all the query samples. However, a caveat here is that the model confidence may be unreliable, which may lead to incorrect predictions. To tackle this issue, we propose to meta-learn the confidence for each query sample, to assign optimal weights to unlabeled queries such that they improve the model's transductive inference performance on unseen tasks. We achieve this by meta-learning an input-adaptive distance metric over a task distribution under various model and data perturbations, which will enforce consistency on the model predictions under diverse uncertainties for unseen tasks. Moreover, we additionally suggest a regularization which explicitly enforces the consistency on the predictions across the different dimensions of a high-dimensional embedding vector. We validate our few-shot learning model with meta-learned confidence on four benchmark datasets, on which it largely outperforms strong recent baselines and obtains new state-of-the-art results. Further application on semi-supervised few-shot learning tasks also yields significant performance improvements over the baselines. The source code of our algorithm is available at https://github.com/seongmin-kye/MCT.

==> self_ensemble2.tex <==
\begin{algorithm}[t!]
  \caption{Transductive inference with self-ensembling}
    \begin{flushleft}
        \textbf{Input:} The number of classes $C$, and the number of transduction steps $T$.
        \\
        \textbf{Input:} The set of support examples $\mathcal{S}^c$, for each class $c=1,\dots,C$.
        \\
        \textbf{Input:} The set of all query examples $\mathcal{Q}_x$.
        \\
        \textbf{Input:} Full-path embedding function $f_\theta$ and drop-layer embedding function $f^\text{drop}_\theta$.
        \\
        \textbf{Input:} Horizontal-flipping operation $\text{Flip}(\cdot)$.
        \\
        \textbf{Output:} Confidence score $q_c^{T}(\btx)$ obtained after $T$ transduction steps, for all $c=1,\dots,C$ and $\btx_i \in \mathcal{Q}_x$.
        \\
    \end{flushleft}
  \begin{algorithmic}[1]
  
    \For{$c = 1,\dots, C$}
    
        \State Compute initial prototype: $P_{0,c} \gets \frac{1}{|\mathcal{S}_c|} \sum_{\bx \in \mathcal{S}_c} f_\theta(\bx)$.
        
        \State \parbox[t]{\dimexpr\textwidth-\leftmargin-\labelsep-\labelwidth}{Repeat with drop-layer (D) embedding function $f^\text{drop}_\theta$ and flipping (F) function $\text{Flip}(\cdot)$ in turn to collect $P_{0,c}, P^{D}_{0,c}, P^{F}_{0,c}, P^{D,F}_{0,c}$.}

    \EndFor
        
    \For{$c = 1,\dots, C$}
        \State Compute initial confidence score: $\rho_{0,ic} \gets \frac{\exp \bigl( -d(\overline{Q}_{i}, \overline{P}_{0,c})/\sigma_{ic}^2\bigr)}
        {\sum_{c'=1}^C \exp\bigl(-d(\overline{Q}_{i}, \overline{P}_{0,c'})/\sigma_{ic'}^2\bigr)}$
        
        \State Repeat with $\{P_{0,c}\}, \{P^{D}_{0,c}\}, \{P^{F}_{0,c}\}, \{P^{D,F}_{0,c}\}$ to collect $\rho_{0,ic}, \rho^{D}_{0,ic}, \rho^{F}_{0,ic}, \rho^{D,F}_{0,ic}$.
        
        \State $q^0_{ic}(\btx) 
        \leftarrow 
        \frac{1}{4}\{\rho_{0,ic} + \rho^{D}_{0,ic} + \rho^{F}_{0,ic} + \rho^{D,F}_{0,ic}\}$ for all $\btx_i \in \mathcal{Q}$.
    \EndFor
    \For{$t=1,\dots, T$}
            \For{$c=1,\dots,C$}
                \State Update class $c$ prototype:  $P_{t,c} \gets \frac{\sum_{\bx_i \in \mathcal{S}^c}1 \cdot S^c_i+\sum_{\btx_i \in \mathcal{Q}_x}q_c^{t-1}(\btx_i) \cdot Q_i}{\sum_{\bx_i \in \mathcal{S}_c}1+\sum_{\btx_i \in \mathcal{Q}_x}q_c^{t-1}(\btx_i)}$.
                
                \State Repeat with $f^\text{drop}_\theta$ and $\text{Flip}(\cdot)$ in turn to collect $\{P_{t,c}, P^{D}_{t,c}, P^{F}_{t,c}, P^{D,F}_{t,c}\}$.
                
            \EndFor
        \For{$c = 1,\dots, C$}
        
            \State Compute $t$-step confidence score: $\rho_{t,c} \gets \frac{\exp \bigl( -d(\overline{Q}_{i}, \overline{P}_{t,c})/\sigma_{ic}^2\bigr)}
            {\sum_{c'=1}^C \exp\bigl(-d(\overline{Q}_{i}, \overline{P}_{t,c'})/\sigma_{ic'}^2\bigr)}$

            \State Repeat with $\{P_{t,c}\}, \{P^{D}_{t,c}\}, \{P^{F}_{t,c}\}, \{P^{D,F}_{t,c}\}$ to collect $\rho_{t,c}, \rho^{D}_{t,c}, \rho^{F}_{t,c}, \rho^{D,F}_{t,c}$.
            
            \State $q^t_{ic}(\btx) 
            \leftarrow 
            \frac{1}{4}\{\rho_{t,c} + \rho^{D}_{t,c} + \rho^{F}_{t,c}
            + \rho^{D,F}_{t,c}\}$  for all $\btx_i \in \mathcal{Q}$
        \EndFor
    \EndFor
  \end{algorithmic}
  \label{algo:transduction}
\end{algorithm}
% \vspace{-0.4in}
% \begin{algorithm}[t!]
%   \caption{Self-Ensembling Transduction (SET)}
%     \begin{flushleft}
%         \textbf{Input:} The number of classes $C$, and the number of transduction steps $T$.
%         \\
%         \textbf{Input:} The set of support examples $\mathcal{S}^c$, for each class $c=1,\dots,C$.
%         \\
%         \textbf{Input:} The set of all query examples $\mathcal{Q}_x$.
%         \\
%         \textbf{Input:} Full-path embedding function $f_\theta$ and drop-layer embedding function $f^\text{drop}_\theta$.
%         \\
%         \textbf{Input:} Horizontal-flipping operation $\text{Flip}(\cdot)$.
%         \\
%         \textbf{Output:} Confidence score $q_c^{T}(\btx)$ obtained after $T$ transduction steps, for all $c=1,\dots,C$ and $\btx_i \in \mathcal{Q}_x$.
%         \\
%     \end{flushleft}
%   \begin{algorithmic}[1]
  
%     \For{$c = 1,\dots, C$}
    
%         \State Compute initial prototype: $P_{0,c} \gets \frac{1}{|\mathcal{S}_c|} \sum_{\bx \in \mathcal{S}_c} f_\theta(\bx)$.
        
%         \State \parbox[t]{\dimexpr\textwidth-\leftmargin-\labelsep-\labelwidth}{Repeat with drop-layer (D) embedding function $f^\text{drop}_\theta$ and flipping (F) function $\text{Flip}(\cdot)$ in turn to collect $P_{0,c}, P^{D}_{0,c}, P^{F}_{0,c}, P^{D,F}_{0,c}$.}

%     \EndFor
        
%     \For{$c = 1,\dots, C$}
%         \State Compute initial confidence score: $\rho_{0,ic} \gets \frac{\exp \bigl( -d(\overline{Q}_{i}, \overline{P}_{0,c})/\sigma_{ic}^2\bigr)}
%         {\sum_{c'=1}^C \exp\bigl(-d(\overline{Q}_{i}, \overline{P}_{0,c'})/\sigma_{ic'}^2\bigr)}$
        
%         \State Repeat with $\{P_{0,c}\}, \{P^{D}_{0,c}\}, \{P^{F}_{0,c}\}, \{P^{D,F}_{0,c}\}$ to collect $\rho_{0,ic}, \rho^{D}_{0,ic}, \rho^{F}_{0,ic}, \rho^{D,F}_{0,ic}$.
        
%         \State $q^0_{ic}(\btx) 
%         \leftarrow 
%         \frac{1}{4}\{\rho_{0,ic} + \rho^{D}_{0,ic} + \rho^{F}_{0,ic} + \rho^{D,F}_{0,ic}\}$ for all $\btx_i \in \mathcal{Q}$.
%     \EndFor
%     \For{$t=1,\dots, T$}
%             \For{$c=1,\dots,C$}
%                 \State Update class $c$ prototype:  $P_{t,c} \gets \frac{\sum_{\bx_i \in \mathcal{S}^c}1 \cdot S^c_i+\sum_{\btx_i \in \mathcal{Q}_x}q_c^{t-1}(\btx_i) \cdot Q_i}{\sum_{\bx_i \in \mathcal{S}_c}1+\sum_{\btx_i \in \mathcal{Q}_x}q_c^{t-1}(\btx_i)}$.
                
%                 \State Repeat with $f^\text{drop}_\theta$ and $\text{Flip}(\cdot)$ in turn to collect $\{P_{t,c}, P^{D}_{t,c}, P^{F}_{t,c}, P^{D,F}_{t,c}\}$.
                
%             \EndFor
%         \For{$c = 1,\dots, C$}
        
%             \State Compute $t$-step confidence score: $\rho_{t,c} \gets \frac{\exp \bigl( -d(\overline{Q}_{i}, \overline{P}_{t,c})/\sigma_{ic}^2\bigr)}
%             {\sum_{c'=1}^C \exp\bigl(-d(\overline{Q}_{i}, \overline{P}_{t,c'})/\sigma_{ic'}^2\bigr)}$

%             \State Repeat with $\{P_{t,c}\}, \{P^{D}_{t,c}\}, \{P^{F}_{t,c}\}, \{P^{D,F}_{t,c}\}$ to collect $\rho_{t,c}, \rho^{D}_{t,c}, \rho^{F}_{t,c}, \rho^{D,F}_{t,c}$.
            
%             \State $q^t_{ic}(\btx) 
%             \leftarrow 
%             \frac{1}{4}\{\rho_{t,c} + \rho^{D}_{t,c} + \rho^{F}_{t,c}
%             + \rho^{D,F}_{t,c}\}$  for all $\btx_i \in \mathcal{Q}$
%         \EndFor
%     \EndFor
%   \end{algorithmic}
%   \label{algo:transduction}
% \end{algorithm}

==> sup_tex/organization.tex <==
\paragraph{Organization} This supplementary file is organized as follows. Section A and B contain detailed descriptions of experimental settings (e.g. datasets, network architectures, hyperparameters and settings for semi-supervised few-shot classification). In Section C, we further explain \emph{Meta-Confidence Transduction} (MCT) in detail. Section D presents more detailed results for the experiments in Figure 4 of main paper. Lastly, we visualize t-SNE embeddings of MCT to show how ensemble confidence affects transduction in Section E.

==> table_tex/ablation_aug_IMS.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\vspace{-0.05in}
 \caption{Ablation study on augmentation strategy on miniImageNet. Every baseline is implemented in prototypical networks with IMS.}
\vspace*{0.03in}
 \begin{tabular}{c c | c c c c }

 \hline
Support & Query & \multicolumn{2}{c}{Inductive} & \multicolumn{2}{c}{Transductive} \\
Aug & Aug & 1-shot & 5-shot & 1-shot & 5-shot \\
 \hline
 \hline



	
	
weak & weak &
58.90\tiny$\pm$0.61 &
74.76\tiny$\pm$0.47 &
67.25\tiny$\pm$0.89 &
76.68\tiny$\pm$0.55	 \\

strong & strong &
59.74\tiny$\pm$0.62 &
75.59\tiny$\pm$0.49 &
69.01\tiny$\pm$0.93 &
78.99\tiny$\pm$0.53	 \\

strong & weak   &
58.09\tiny$\pm$0.64 &
74.03\tiny$\pm$0.48 &
67.94\tiny$\pm$0.88 & 
77.24\tiny$\pm$0.55 \\

weak & strong   &
61.08\tiny$\pm$0.66 &
77.26\tiny$\pm$0.46 &
69.45\tiny$\pm$0.86 & 
79.54\tiny$\pm$0.54 \\
\hline
 \end{tabular}
 \vspace{-0.15in}
 \label{tbl:ablation_aug_IMS}
\end{table*}


==> table_tex/ablation_aug_PMS.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\vspace{-0.05in}
 \caption{Ablation study on augmentation strategy on miniImageNet. Every baseline is implemented in prototypical networks with PMS.}
\vspace*{0.03in}
 \begin{tabular}{c c | c c c c }

 \hline
Support & Query & \multicolumn{2}{c}{Inductive} & \multicolumn{2}{c}{Transductive} \\
Aug & Aug & 1-shot & 5-shot & 1-shot & 5-shot \\
 \hline
 \hline
weak & weak &
58.21\tiny$\pm$0.61 & 75.99\tiny$\pm$0.52 &
64.43\tiny$\pm$0.62 & 78.49\tiny$\pm$0.50 \\

strong & strong &
60.93\tiny$\pm$0.65 & 76.59\tiny$\pm$0.45 &
69.55\tiny$\pm$0.71 & 79.15\tiny$\pm$0.52 \\

strong & weak   &
56.75\tiny$\pm$0.64 & 74.32\tiny$\pm$0.50 &
66.12\tiny$\pm$0.60 & 75.71\tiny$\pm$0.52 \\

weak & strong   &
\textbf{61.81\tiny$\pm$0.58} &
\textbf{77.67\tiny$\pm$0.50} &
\textbf{71.95\tiny$\pm$0.81} & 
\textbf{81.06\tiny$\pm$0.51} \\
\hline
 \end{tabular}
 \vspace{-0.15in}
 \label{tbl:ablation_aug_PMS}
\end{table*}


==> table_tex/main_result.tex <==
% \begin{tabular}{c c c c c c c c c c c c}
\begin{table*}[t!]
\centering
\tiny
\vspace{-0.05in}
\caption{\small \textbf{Average classification performance} over 1000 randomly generated episodes, with 95\% confidence intervals. We consider 5-way classification on all the datasets. $^*$ denotes it is reported from \cite{DPGN}. $\dagger$ indicates the transductive inference with top-$k$ selection method introduced by \cite{hou2019cross}.}
\vspace*{0.03in}
 \begin{tabularx}{\textwidth}{
 c @{\extracolsep{\fill}} 
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}
 c @{\extracolsep{\fill}}}
 
 \hline
& \multirow{2}{*}{Model}  &
\multirow{2}{*}{Backbone} &
\multicolumn{2}{c}{miniImageNet}& \multicolumn{2}{c}{tieredImageNet}&
\multicolumn{2}{c}{CIFAR-FS} &
\multicolumn{2}{c}{FC100} \\
 &  &  & 1-shot & 5-shot & 1-shot & 5-shot &
 1-shot & 5-shot & 1-shot & 5-shot\\
 \hline
 \hline
\multirow{7}{*}{\textbf{I}}&
MTL$^{*}$~\cite{MTL} & ResNet-12 &
61.20\tiny$\pm$1.80 & 75.53\tiny$\pm$0.80 &
65.62\tiny$\pm$1.80 & 80.61\tiny$\pm$0.90 &
- & - &
- & - \\

& TapNet~\cite{yoon2019tapnet} & ResNet-12    & 61.65\tiny$\pm$0.15 & 76.36\tiny$\pm$0.10 & 63.08\tiny$\pm$0.15 & 80.26\tiny$\pm$0.12 &
-&-&-&-\\

&TADAM~\cite{oreshkin2018tadam} & ResNet-12    &
58.56\tiny$\pm$0.39 & 76.65\tiny$\pm$0.38 &
62.13\tiny$\pm$0.31 & 81.92\tiny$\pm$0.30 &
- & - &
40.1\tiny$\pm$0.4 & 56.1\tiny$\pm$0.4 \\

% &TADAM+AM3~\cite{TADAM2} & ResNet-12    &
% \textbf{65.30\tiny$\pm$0.49} &
% 78.10\tiny$\pm$0.36 &
% 69.08\tiny$\pm$0.47 &
% 82.58\tiny$\pm$0.31 &
% - & - & - & - \\

& MetaOpt-SVM~\cite{lee2019meta} & ResNet-12    & 62.64\tiny$\pm$0.61 & 78.63\tiny$\pm$0.46 & 65.99\tiny$\pm$0.72 & 81.56\tiny$\pm$0.53 & 72.00\tiny$\pm$0.70 & 84.20\tiny$\pm$0.50 & 41.10\tiny$\pm$0.60 &  55.50\tiny$\pm$0.60\\

& Dense~\cite{lifchitz2019dense}  & ResNet-12    & 61.26\tiny$\pm$0.20 & 79.01\tiny$\pm$0.13 &
- & - & - & - & 
42.04\tiny$\pm$0.17 & 57.05\tiny$\pm$0.16\\

& CAN~\cite{hou2019cross} & ResNet-12    & 63.85\tiny$\pm$0.48 &
79.44\tiny$\pm$0.34 & 
\textbf{69.89\tiny$\pm$0.51} &
84.23\tiny$\pm$0.37 &
-&-&-&-\\
& IMS+DC & ResNet-12    & 
\textbf{64.81\tiny$\pm$0.65} &
\textbf{81.31\tiny$\pm$0.45} &
\textbf{69.37\tiny$\pm$0.69} &
\textbf{84.96\tiny$\pm$0.48} &
75.67\tiny$\pm$0.69 &
88.32\tiny$\pm$0.44 &
43.47\tiny$\pm$0.58 &
58.97\tiny$\pm$0.58 \\
& IMS+DC+Aug & ResNet-12 & 
\textbf{65.34\tiny$\pm$0.63} &
\textbf{82.15\tiny$\pm$0.45} &
\textbf{69.66\tiny$\pm$0.72} &
\textbf{85.29\tiny$\pm$0.49} &
\textbf{77.84\tiny$\pm$0.64} &
\textbf{89.11\tiny$\pm$0.45} &
\textbf{44.69\tiny$\pm$0.60} &
\textbf{60.33\tiny$\pm$0.59} \\
\hline
% \textbf{64.49\tiny$\pm$0.64} &
% \textbf{81.63\tiny$\pm$0.44} &
% 68.41\tiny$\pm$0.73 &
% \textbf{84.60\tiny$\pm$0.50}&
% \textbf{76.23\tiny$\pm$0.67}&
% \textbf{88.39\tiny$\pm$0.44}&
% \textbf{43.01\tiny$\pm$0.58}&
% \textbf{59.67\tiny$\pm$0.56}\\
% \hline

\multirow{10}{*}{\textbf{T}} & TPN~\cite{liu2018learning} & ConvNet-64   & 55.51\tiny$\pm$0.86 &
69.86\tiny$\pm$0.65 & 59.91\tiny$\pm$0.94 & 73.30\tiny$\pm$0.75 
&-&-&-&-\\
& EGNN$^{*}$~\cite{kim2019edge} & ConvNet-256  &
59.63\tiny$\pm$0.52  & 76.34\tiny$\pm$0.48  &
63.52\tiny$\pm$0.52  & 80.24\tiny$\pm$0.49  &   
-&-&-&-\\
& TEAM~\cite{trans_episodic} & ResNet-18    &
60.07 & 75.90 &
- & - &
-&-&-&-\\
& MAML+SCA~\cite{SCA} & DenseNet  &
62.86\tiny$\pm$0.79 & 77.46\tiny$\pm$1.18 &
- & - &
- & - &
- & - \\
& Fine-tuning~\cite{baseline} & WRN-28-10  &
65.73\tiny$\pm$0.68 & 78.40\tiny$\pm$0.52 &
73.34\tiny$\pm$0.71 & 85.50\tiny$\pm$0.50 &
76.58\tiny$\pm$0.68 & 85.79\tiny$\pm$0.50 &
43.16\tiny$\pm$0.59 & 57.57\tiny$\pm$0.55 \\
& SIB~\cite{SIB} & WRN-28-10  &
70.0\tiny$\pm$0.6 & 79.2\tiny$\pm$0.4 &
- & - &
80.0\tiny$\pm$0.6 & 85.3\tiny$\pm$0.4 &
-&-\\
& CAN + Top-$k^\dagger$~\cite{hou2019cross} & ResNet-12    & 67.19\tiny$\pm$0.55 & 80.64\tiny$\pm$0.35 &
73.21\tiny$\pm$0.58 & 84.93\tiny$\pm$0.38 &
-&-&-&-\\
& DPGN~\cite{DPGN} & ResNet-12    &
67.77\tiny$\pm$0.32 &
84.60\tiny$\pm$0.43 &
72.45\tiny$\pm$0.51 &
\textbf{87.24\tiny$\pm$0.39} &
77.90\tiny$\pm$0.50 &
\textbf{90.20\tiny$\pm$0.40} &
-&-\\
& IMS+DC+MCT  & ResNet-12    &
76.65\tiny$\pm$0.84 &
85.09\tiny$\pm$0.43 &
81.19\tiny$\pm$0.87 &
\textbf{86.94\tiny$\pm$0.50} &
85.61\tiny$\pm$0.69 &
\textbf{89.97\tiny$\pm$0.45} &
49.61\tiny$\pm$0.82 &
61.68\tiny$\pm$0.61 \\
& IMS+DC+MCT+Aug  & ResNet-12    &
\textbf{78.55\tiny$\pm$0.86} &
\textbf{86.03\tiny$\pm$0.42} &
\textbf{82.32\tiny$\pm$0.81} &
\textbf{87.36\tiny$\pm$0.50} &
\textbf{87.14\tiny$\pm$0.72} &
\textbf{90.62\tiny$\pm$0.46} &
\textbf{51.16\tiny$\pm$0.88} &
\textbf{63.28\tiny$\pm$0.61} \\
\hline
 \end{tabularx}
 \vspace{-0.1in}
 \label{tbl:main_result}
\end{table*}
